Attention over learned object embeddings enables complex visual reasoning

Neural networks have achieved success in a wide array of perceptual tasks but often fail at tasks involving both perception and higher-level reasoning. On these more challenging tasks, bespoke approaches (such as modular symbolic components, independent dynamics models or semantic parsers) targeted towards that specific type of task have typically performed better. The downside to these targeted approaches, however, is that they can be more brittle than general-purpose neural networks, requiring significant modification or even redesign according to the particular task at hand. Here, we propose a more general neural-network-based approach to dynamic visual reasoning problems that obtains state-of-the-art performance on three different domains, in each case outperforming bespoke modular approaches tailored specifically to the task. Our method relies on learned object-centric representations, self-attention and self-supervised dynamics learning, and all three elements together are required for strong performance to emerge. The success of this combination suggests that there may be no need to trade off flexibility for performance on problems involving spatio-temporal or causal-style reasoning. With the right soft biases and learning objectives in a neural network we may be able to attain the best of both worlds.

==> clevrer_examples.tex <==
% Auto-generated by pick_clevrer_examples.py

%%%%%%%%%%%%%%%%%%

  \includegraphics[width=1.1\textwidth]{clevrer_videos/video2564.png}
  \begin{tabular}{c|c|c|c}
  
  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} What material is the last object to collide with the rubber cylinder? \\
  \textbf{Model:} rubber \\
  \textbf{Label:} rubber\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} Which of the following is responsible for the metal cube's colliding with the sphere?
  \begin{enumerate}[leftmargin=*]
  \item the presence of the blue cube
\item the red cube's colliding with the cylinder
\item the presence of the cylinder
  \end{enumerate}
  \textbf{Model:} 2, 3 \\
  \textbf{Label:} 2, 3\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} What will happen next?
  \begin{enumerate}[leftmargin=*]
  \item The metal cube and the sphere collide
\item The blue cube collides with the sphere
  \end{enumerate}
  \textbf{Model:} 2 \\
  \textbf{Label:} 2\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} What will not happen if the sphere is removed?
  \begin{enumerate}[leftmargin=*]
  \item The cylinder collides with the blue object
\item The red cube collides with the cylinder
\item The metal object collides with the blue cube
  \end{enumerate}
  \textbf{Model:} 3 \\
  \textbf{Label:} 3\\
  \end{minipage}
  \\ 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} How many red objects enter the scene? \\
  \textbf{Model:} 1 \\
  \textbf{Label:} 2\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} Which of the following is responsible for the metal cube's colliding with the sphere?
  \begin{enumerate}[leftmargin=*]
  \item the presence of the blue cube
\item the red cube's colliding with the cylinder
\item the presence of the cylinder
  \end{enumerate}
  \textbf{Model:} 2, 3 \\
  \textbf{Label:} 2, 3\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} What will happen next?
  \begin{enumerate}[leftmargin=*]
  \item The metal cube and the sphere collide
\item The blue cube collides with the sphere
  \end{enumerate}
  \textbf{Model:} 1, 2 \\
  \textbf{Label:} 2\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} If the rubber cube is removed, which of the following will happen?
  \begin{enumerate}[leftmargin=*]
  \item The metal cube collides with the cylinder
\item The cylinder and the sphere collide
  \end{enumerate}
  \textbf{Model:} 1 \\
  \textbf{Label:} 1, 2\\
  \end{minipage}
  
  \end{tabular}
  

%%%%%%%%%%%%%%%%%%

  \includegraphics[width=1.1\textwidth]{clevrer_videos/video2396.png}
  \begin{tabular}{c|c|c|c}
  
  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} How many moving red objects are there when the video ends? \\
  \textbf{Model:} 1 \\
  \textbf{Label:} 1\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} Which of the following is responsible for the rubber cube's colliding with the sphere?
  \begin{enumerate}[leftmargin=*]
  \item the collision between the gray cube and the cylinder
\item the presence of the brown metal cylinder
\item the metal cube's entering the scene
  \end{enumerate}
  \textbf{Model:} 1, 2 \\
  \textbf{Label:} 1, 2\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} What will happen next?
  \begin{enumerate}[leftmargin=*]
  \item The sphere collides with the metal cube
\item The rubber cube and the metal cube collide
  \end{enumerate}
  \textbf{Model:} 2 \\
  \textbf{Label:} 2\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} If the red cube is removed, what will happen?
  \begin{enumerate}[leftmargin=*]
  \item The rubber cube and the cylinder collide
\item The cylinder and the sphere collide
\item The gray object collides with the sphere
  \end{enumerate}
  \textbf{Model:} 1, 2, 3 \\
  \textbf{Label:} 1, 2, 3\\
  \end{minipage}
  \\ 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} What color is the object to collide with the sphere? \\
  \textbf{Model:} gray \\
  \textbf{Label:} gray\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} Which of the following is responsible for the rubber cube's colliding with the sphere?
  \begin{enumerate}[leftmargin=*]
  \item the collision between the gray cube and the cylinder
\item the presence of the brown metal cylinder
\item the metal cube's entering the scene
  \end{enumerate}
  \textbf{Model:} 1, 2 \\
  \textbf{Label:} 1, 2\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} What will happen next?
  \begin{enumerate}[leftmargin=*]
  \item The sphere collides with the metal cube
\item The rubber cube and the metal cube collide
  \end{enumerate}
  \textbf{Model:} 2 \\
  \textbf{Label:} 2\\
  \end{minipage}
  & 

  \begin{minipage}[t]{0.245\textwidth}
  \textbf{Q:} If the gray cube is removed, which of the following will happen?
  \begin{enumerate}[leftmargin=*]
  \item The cylinder and the red object collide
\item The cylinder collides with the sphere
  \end{enumerate}
  \textbf{Model:} 2 \\
  \textbf{Label:} 2\\
  \end{minipage}
  
  \end{tabular}
  
